Learning from Pseudo-labeled Segmentation for Multi-Class Object Counting

Class-agnostic counting (CAC) has numerous potential applications across various domains. The goal is to count objects of an arbitrary category during testing, based on only a few annotated exemplars. In this paper, we point out that the task of counting objects of interest when there are multiple object classes in the image (namely, multi-class object counting) is particularly challenging for current object counting models. They often greedily count every object regardless of the exemplars. To address this issue, we propose localizing the area containing the objects of interest via an exemplar-based segmentation model before counting them. The key challenge here is the lack of segmentation supervision to train this model. To this end, we propose a method to obtain pseudo segmentation masks using only box exemplars and dot annotations. We show that the segmentation model trained on these pseudo-labeled masks can effectively localize objects of interest for an arbitrary multi-class image based on the exemplars. To evaluate the performance of different methods on multi-class counting, we introduce two new benchmarks, a synthetic multi-class dataset and a new test set of real images in which objects from multiple classes are present. Our proposed method shows a significant advantage over the previous CAC methods on these two benchmarks.

==> bakup.tex <==
\begin{table*}[!ht] 
  \centering
\resizebox{0.72\textwidth}{!}{%
  \begin{tabular}{l|c|cccc|cccc}
    \toprule
   \multirow{2}{*}{Method} & \multirow{2}{*}{Input} & \multicolumn{4}{c|}{Val Set} & \multicolumn{4}{c}{Test Set} \\
    & & MAE & RMSE & NAE & SRE & MAE & RMSE & NAE & SRE \\
    \midrule
    %\multirow{2}{*}{GMN \cite{Lu2018CAC}} & GT & {29.66} & {89.81} & - & - & {26.52} & {124.57} & - & - \\
    %& RPN & {40.96} & {108.47} & - & - & {39.72} & {142.81} & - & - \\
    %\midrule
    %\multirow{2}{*} {FamNet} & GT & {24.32} & {70.94} & {22.56} & {101.54} \\
    % & RPN & {48.62} & {120.77} & {53.82} & {155.38}  \\
    %\midrule
    \multirow{2}{*}{FamNet+ \cite{Ranjan2021LearningTC}} & w/o concatenation & {23.75} & {69.07} & 0.52 & 4.25 & {22.08} & {99.54} & 0.44 & 6.45 \\
     & w/ concatenation & {27.83} & {39.79} & 1.33 & 7.30 & {32.10} & {57.20}  & 1.16 & 8.86 \\
     \midrule
     \multirow{2}{*}{BMNet \cite{Shi2022SimiCounting}} & w/o concatenation & {19.46} & {72.35} & 0.26 & 3.31 & {18.18} & {123.76} & 0.26 & 4.16 \\
     & w/ concatenation & 32.54 & 46.03 & 1.76 & 9.87 & 40.45 & 75.76 & 1.64 & 9.65 \\
     \midrule
    \multirow{2}{*} {BMNet+ \cite{Shi2022SimiCounting}} & w/o concatenation & 15.73 & 58.52 & 0.25 & 2.72 & 14.62 & 91.83 & 0.27 & 6.20  \\
     & w/ concatenation & 31.07 & 42.42 & 1.74 & 9.51 & 40.98 & 59.38 & 1.79 & 11.94 \\
    \midrule
    %{FamNet} & {32.15} & {98.75} & {32.27} & {131.46} \\
    %{BMNet} & & {34.09} & {105.05} & {31.27} & {124.85} \\
    %{BMNet+} & & {35.15} & {106.07} & {34.52} & {132.64} \\
    %{BMNet+} & {23.01} & {72.61} & {22.43} & {128.12} \\
    \multirow{3}{*}{Ours (Base)} & w/o concatenation & {18.55} & {61.12} & 0.30 & 3.18 & {20.68} & {109.14} & 0.36 & 7.63 \\
     & w/ concatenation & 32.69 & 45.29 & 1.83 & 10.16 &  44.89 & 69.85 & 1.94 & 12.91  \\
     & Patch-Seg & \textbf{14.46} & \textbf{26.05} & \textbf{0.62} & \textbf{4.49} & \textbf{15.40} & \textbf{63.82} & \textbf{0.43} & \textbf{3.68} \\
    \bottomrule
  \end{tabular}} \\ \vspace{3mm}
  \caption{ Quantitative comparisons on FSC-147 dataset. ``GT" denotes using human-annotated boxes as exemplars. ``RPN" denotes using top-3 RPN proposals with highest objectness scores as exemplars. ``Patch-Selection" denotes using our selected patches as exemplars.
  }\label{tab:test_val}%
\end{table*}



\begin{table*}[!ht] 
  \centering
\resizebox{0.83\textwidth}{!}{%
  \begin{tabular}{l|c|cccc|cccc}
    \toprule
   \multirow{2}{*}{Method} & Training & \multicolumn{4}{c|}{Multi Set} & \multicolumn{4}{c}{Single Set} \\
    & Set & Val MAE & Val RMSE & Test MAE & Test RMSE & Val MAE & Val RMSE & Test MAE & Test RMSE   \\
    \midrule
    \multirow{2}{*}{BMNet+} & Single & {31.09} & {42.43} & 39.78 & 57.85 & 15.74 & 58.53 & 14.62 & 91.83 \\
    & Single+Multi & 17.64  & {26.24} & 20.57 & 34.60 & 22.87 & 76.68 & 20.94 & 103.40 \\
    \midrule
    \multirow{2}{*}{FamNet+ \cite{Ranjan2021LearningTC}} & Single & {27.74} & {39.78} & 29.90 & 43.59 & 23.75 & 69.07 & 22.08 & 99.54 \\
     & Single+Multi & {16.97} & {28.44} & 20.34 & 28.66 &  29.45 & 94.33 & 26.93 & 116.12 \\
     %\midrule\multirow{2}{*}{SAFECount \cite{Ranjan2021LearningTC}} & Single & {22.58} & {34.68} & 26.44 & 40.68 & 14.42 & 69.07 & 22.08 & 99.54 \\
     %& Single+Multi & {16.97} & {28.44} & 20.34 & 28.66 &  29.45 & 94.33 & 26.93 & 116.12 \\
     %\multirow{2}{*}{BMNet \cite{Shi2022SimiCounting}} & GT & {18.29} & {124.02} & 0.26 & 4.39  \\
     %& RPN & {37.26} & {108.54} & {0.42} & {5.43}  \\
     %\midrule
    %\multirow{2}{*} {BMNet+ \cite{Shi2022SimiCounting}} & GT & {14.68} & {91.74} & {0.27} & {6.57}  \\
     %& RPN & {35.15} & {106.07} & {0.41} & {5.28}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{1mm}
  \caption{ Quantitative comparisons on FSC-147 dataset. ``GT" denotes using human-annotated boxes as exemplars. ``RPN" denotes using top-3 RPN proposals with highest objectness scores as exemplars. ``Patch-Selection" denotes using our selected patches as exemplars.
  }\label{tab:test_val}%
\end{table*}


Due to this trade-off, we believe a better strategy for multi-class counting is to localize the target area first and then count only the objects inside this area. 
%only and the counting can be accomplished via a single-class counting model. 
%In this way, the counting model does not need to sacrifice the performance on single-class counting in order to perform multi-class counting.
%To this end, we build a segmentation model that can segment objects of interest given only a few annotated exemplars. Some closely related tasks include unsupervised semantic segmentation, zero/few-shot semantic segmentation, \etc. However, the goal of these tasks is to assign a semantic label to each pixel in the image. They usually require a large amount of training data (either annotated or not) and the label space is limited to a set of pre-defined categories. In comparison, our goal is to simply localize the region of interest specified by a few exemplars, which can belong to an arbitrary class. 
% limited to a specific dataset/domain, pre-defined label space
In particular, given a multi-class input image, a few annotated exemplars, and a pre-trained single-class counting model, our goal is to compute a coarse mask that can be applied on the feature maps of the counting model to exclude the non-target area. 
The mask is at a lower resolution than the input image and each pixel in the mask corresponds to an image patch.
Our goal is to assign a binary label to each mask pixel indicating if the corresponding image patch contains the object of interest or not. To do this, we first use a pre-trained feature extractor to extract the embeddings of the annotated exemplars and compute their average to construct a prototype.
Then for each pixel in the mask, we find the corresponding image patch and extract its feature embedding. 
%Then we extract the embeddings for a set of image patches, each of which corresponds to a pixel in the mask.
We combine all the extracted patch embeddings with the pre-computed prototype and run $K$-means on them. Those patches whose embeddings fall into the same cluster as the prototype will be considered to contain the object of interest and vice versa.
%and results in a 1 value in the corresponding mask pixel. 

In particular, given a synthetic multi-class image, a few annotated exemplars, and a pre-trained single-class counting model, our goal is to compute a coarse segmentation mask that can be used to exclude the non-target area from the similarity maps of the counting model.  
Each pixel of this mask will be assigned a binary label indicating if it contains the objects of interest or not. To do this, we first crop a set of image patches, each of which corresponds to a pixel on the mask. 
Then we extract the feature embeddings for all these image patches as well as the provided exemplars and run $K$-Means clustering on them. Those patches whose embeddings fall into the same cluster as the provided exemplar will be considered to contain the object of interest, which results in a positive label in the corresponding mask pixel, and vice versa.

 In particular, we first associate each mask pixel with an image patch based on the receptive field of the network. We aim to assign a binary label to each pixel indicating if the corresponding patch contains the objects of interest or not. To do this, we extract the feature embeddings for all the cropped patches as well as the provided exemplars and run $K$-Means clustering on them. Those patches whose embeddings fall into the same cluster as the exemplar will be considered to contain the object of interest, which results in a positive label in the corresponding mask pixel, and vice versa.

 The above strategy allows us to obtain segmentation masks from exemplars in an intuitive and straightforward way. However, it is worth noting that the number of clusters, denoted as $K$, has a large effect on the output binary mask and the final counting results.
%However, determining the number of clusters, $K$, for an arbitrary image is non-trivial as the number of object classes present in the image is unknown. 
If $K$ is too small, too many patch embeddings will fall into the same cluster as the exemplar and the counter will over-count the objects; if $K$ is too big, too few embeddings will fall into the same cluster, which results in too many regions being masked out. In order to choose $K$'s optimal value, we propose to find the $K$ such that after applying the corresponding binary mask, the counting model can produce a density map closest to the ground truth map. In this way, we can obtain the optimal masks for all the training images and then train an exemplar-based segmentation model to approximate them. 
%Thus, instead of running $K$-Means during testing, 
%we first find the optimal $K$ for each training image that leads to the best binary mask. Then we use this optimal mask as the supervision signal to train a segmentation model based on the provided exemplar box. 
%we first find the optimal $K$ for each image in the multi-class training set that leads to the best binary mask. Then we train a segmentation model to predict this mask based on the provided exemplar box. 
The trained segmentation model can then be used to predict the mask for an arbitrary testing image.


We thank all the reviewers for their time and valuable comments! We are very encouraged to see that reviewers agree that our proposed task is useful and the method is novel and interesting with extensive experiments and strong results.  %and the results are strong (\rtwo,\rthree). 
%The main concerns of the reviewers are at the NLP model: 
We address the major concerns below:

\qu{(\rone)} {Results on other counting datasets.} We tested our method on the COCO subset proposed in CFOCNet (Yang \etal 2021) - see Tab. \ref{tab:coco}. We will include this experiment.
\begin{table}[!h] 
\vspace{-10pt}
  \centering
\resizebox{0.495\textwidth}{!}{%
  \begin{tabular}{c|cc|cc}
    \toprule
    & MAE (N $\geq$1) & RMSE (N $\geq$1) & MAE (N $\geq$5) & RMSE (N $\geq$5) \\
    \midrule
    %CFOCNet (1-shot) & {2.16} & {3.27} & {3.19} & {4.40}  \\ 
    CFOCNet (5-shot) & \textbf{1.90} & \textbf{2.80} &  {2.82} & {3.77}  \\
    Ours (0-shot) & {2.51} & {3.15} &  \textbf{2.53} & \textbf{3.17}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{1pt}
  \caption{ COCO subset. $N$ is the number of instances in the image.
  } \vspace{-15pt} \label{tab:coco}
\end{table}

\qu{(\rone)} {No ablation study on the number of exemplars.} We show in Tab. \ref{tab:num_k} the performance when using different number of exemplars. We observe that there is no significant performance difference. We use $3$ exemplars in the experiments to be consistent with recent counting methods [29,33] and thus directly comparable with them.
%for keeping consistent with the base counting model.
\begin{table}[!h] 
\vspace{-10pt}
  \centering
\resizebox{0.35\textwidth}{!}{%
  \begin{tabular}{c|ccccc}
    \toprule
    %Number of  & \multicolumn{2}{c|}{Val Set} & \multicolumn{2}{c}{Test Set} \\
    \#Exemplars & 1 & 2 & 3 & 4 & 5\\
    \midrule
    MAE & {27.54} & {27.10} & \textbf{26.93} & {26.99} & 26.97 \\ 
    MSE & {89.45} & \textbf{88.44} &  {88.63} & {88.59} & 88.58 \\
    %3 & \textbf{26.93} & {88.63} &  {22.09} & {115.17}  \\
    %4 & {26.99} & {88.59} &  {22.42} & {115.32}  \\
    %5 & {26.97} & {88.58} &  {22.79} & {116.01}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{2pt}
  \caption{ Performance when using different numbers of exemplars. 
  } \vspace{-14pt} \label{tab:num_k}
\end{table}

\qu{(\rone)}{How does the error predictor perform?} We use the trained error predictor to estimate the counting error for $2000$ patches sampled from $200$ testing images. On average, the estimated error is within $\pm24.9\%$ of the actual counting error. 
\qu{(\rone)} {Why having humans in the loop is not practical for anomaly detection systems?} %We will adjust the language to reflect that surveillance systems often operate perpetually, which is costly to involve humans in the loop.  
Here we refer to surveillance systems that can detect anomalies automatically. We will clarify this.
\qu{(\rone)}{Is this error predictor idea existed in other ZSL works?} 
To the best of our knowledge, we are the first to propose this error predictor and show its effectiveness for ZSL task.
\qu{(\rone)}{Why we need both $F(I)$ and $S$ as inputs?} We adopt this strategy from [29] and [33]. The similarity map highlights the object locations while the exact object counts are estimated from the image features.

\qu{(\rtwo)}{Why the prototype should be an ImageNet feature?} We use ImageNet features since they are class-discriminative, which is helpful to find patches that belong to the same class as the prototype. 
Further, by using ImageNet features, the exemplar selection is independent of the counting network and thus applicable to other exemplar-based methods, as shown in Sec. 5.2.
%compared with counting feature.
%i.e., features close to each other belong to the same class.
%This allows us to find accurate class-relevant patches by selecting the $k$-nearest neighbors of the prototype. 
%(ii) there appears to be no link between the exemplar and the final trained features of the base model (or at least it is not clear if the final features are frozen at their ImageNet initialization); 
%\qu{(\rtwo)}{No link between the exemplar and the final trained features?} We clarify that we use ImageNet to find exemplars., we extract their features using the counting network to compute the similarity map for counting.
%\qu{(\rtwo)}{Are the final features ImageNet?}
\qu{(\rtwo)}{No link between the exemplar and the final trained features.} We clarify that when selecting class-relevant patches, we use ImageNet features. When counting, we use the base counting model to extract features for the exemplars. This base counting model is initialized from pre-trained ImageNet model and then trained with the counting loss. 
%When selecting class-relevant patches, we use ImageNet features. The exemplar features from the base counting model are not frozen and are supervised by the counting loss.
%When selecting class-relevant patches, we use ImageNet features that are frozen after initialization to ensure discriminability. The exemplar features from the base counting model are not frozen and are supervised by the counting loss.
\qu{(\rtwo)}{How the VAE is conditioned on the text embedding?} %We first concatenate the text embedding ($512$-d vector) with the input feature and input them into the encoder of the VAE. We then take the output of the encoder, concatenate it with the text embedding and input them to the decoder. 
We follow the CVAE model (Sohn \etal 2015) to concatenate the text embedding to both the input feature and the latent code.
\qu{(\rtwo)} {Clarify details of the networks and modules.} The prototype generation module is the decoder of the VAE, which is a two-layer FC network with $4096$ hidden units. %We use the decoder to generate $500$ features for each class and take the mean feature as the class prototype. 
%We select the patches whose embeddings are the $k$-nearest neighbors of the prototype as class-relevant patches. 
The error predictor for patch selection is composed of $5$ convolutional layers with ReLU as activation functions. They are followed with a linear layer of size $25 \times 1$. We will change the ``a few" in Lines 491 and 499 to ``$5$" in the revision.
We will also publish the code to ensure reproducibility. \qu{(\rtwo)} {A few corrections and suggested improvements.} Thanks for these suggestions! We will correct them carefully. 

\qu{(\rthree)}{%The patch selection mechanism is not well studied. 
Using zero-shot instance segmentation (ZSI) or selective search (SS) may produce more instance-aware proposals and better results.} 
%Thanks for the insightful comments. It is also our intuitive idea that the proposals should be more instance-aware and we compared random proposals with RPN proposals (S.M. Sec. 3). We also show the results of selective search and ZSI in Tab. \ref{tab:candi_patches}. 
We indeed had the same thought. We first refer to our experiment in S.M. Sec. 3 where we use RPN proposals instead of random crops (which are more instance-aware). Further, we also try ZSI (Zheng \etal 2021) and selective search as suggested (Tab. \ref{tab:candi_patches}).
Surprisingly, we find that the results are not significantly different. We believe this is because the current dataset is relatively simple, i.e., images mostly contain visually similar objects appearing repetitively. Thus, exemplars containing some repetitive patterns can be sufficient for the model to output reasonably accurate counts. %Instance-aware proposals do not yield significant advantages.
We hypothesize that for more complex datasets, more instance-aware proposals might prove advantageous.
%Since the current dataset is very simple, the counter might only need to learn some repetitive patterns to perform counting rather than the perfect object crop. Thus, instance-aware proposals do not yield significant advantages for the counter. We believe for other complicated datasets, instance-aware proposals will bring more benefits. %Please note that our patch selection method can be built on top of any type of proposals.% We will include these results in our revised version.
%Thanks for the suggestion. We report the performance of using RPN proposals in SM. We also apply selective search and ZSI to obtain candidate proposals as suggested. Results are summarized in Tab. \ref{tab:candi_patches}. We observe that ZSI or RPN proposals are indeed more instance-aware. However, the counting performance is not significantly better compared with using random selected patches.   

%\qu{\rthree}{if the selection was good, the predictor wouldn't be necessary.}
%\qu{\rthree}{explore the actual selection further}

%The biggest weakness I found in this paper is also its main contribution: the patch selection mechanism. I really like the idea and it provides reasonable results, but I truly don't think that the solution presented in this paper is yet well studied and I see a lot of potential in continuing this investigation/experimentation before publishing this manuscript. For example, as shown in Figure 5, k-means over the random patches produces pretty arbitrary and unsatisfactory top-10 class-relevant patches. The authors in line 645 claims that "all 10 patches exhibit class specific features", but that's rather obvious: the whole image practically contains "chicken wings". However, the actual selected patches are not well centered on individual instances, which reduces the overall exemplar potential (and the novelty of this paper, imho). Table 2 also shows the limited benefit of the prototype selection, likely due to this random patches + k-means problem. The authors somehow mitigate this problem by introducing a Predictor, which selects the subset of prototypes that are actually good (i.e., those that capture the instance, if present, otherwise it fails). I think the idea of error count prediction is interesting, but it is necessary to fix a problem introduced by a weak selection design. If the selection was good, the predictor wouldn't be necessary. My suggestion to the authors is to explore the actual selection further, as it can lead to substantially better exemplar and eventually better counting performance. For example, why not use zero-shot instance segmentation techniques to generate patches that are more instance-aware (as opposed to random). Without going into the latest advances of zero-shot instance segmentation, even the old selective search proposals (CVPR 2011) would likely produce much better patch proposals.



%Because of the random patch proposal (followed by k-means and top-10 procedure), I also have concerns about the usability of such technique in the wild/actual real problems. For example, what happens when there are only 1 or 2 instances of a specific object in a crowed image? Would this technique still work (ie., how likely will random patches cover this rare instances and how reliably would the k-mean pick those)? For example, would the proposed method be able to count the number of forks in the last figure of Fig. 2 in the supplementary material? The paper presents results on a single dataset of very simple images, but it needs a deeper investigation in more realistic scenarios.
\qu{\rthree}{Would random crops work for images with a few object instances? }
%We agree. 
We indeed cannot guarantee it will always pick up one of the instances. 
%Here we consider random cropping as the simplest form of proposals.
For these cases, other types of proposals (SS, RPN or ZSI) can be better choices. They can directly be used with our method.
%Our method can be built on top of them as well. 
%While our method works well with random cropping, it can be used with any advanced methods such as RPN, SS, or ZSI. 
%For example, counting forks in the last image of Fig.2 - S.M. 
%Note that our method can be built on top of any type of object proposal. %e.g., RPN. 
%We observe that the naive patch sampling works sufficiently well at scanning all possible objects. 
%\qu{\rthree}{Counting for images with only 1-2 object instances (last image in Fig.2 - S.M.?} For the most part, our model can handle well these cases (it outputs 3 forks when simply using random crops). 
%\qu{\rthree}{Counting for images with only 1-2 object instances}
\qu{\rthree}{More ablations studies on parameters.} We conduct ablation studies on the number of exemplars/proposals/class-relevant patches. The results are shown in Tab. \ref{tab:num_k}. %Our method is not sensitive to the choice of hyper-parameters.


%To my understanding, the error predictor learns a general distribution of how objects appear within an image. What if a new image has a considerably different density and displacement? Would the model be able to deal with such a change?
%What happens if the image in Fig. 3 has grapes of different colors (e.g., yellow and red grape)? Would the prototype generate cover both of those? Is there a risk that biases in the generator will lead to biases in the selection (i.e., some instance types are never counted)?

%\qu{\rthree}{Will the model deal with images with different densities?} 
\qu{\rthree}{Generalizing to different object densities and placements.} %As a data-driven method, we cannot guarantee generalizability beyond the patterns exhibited in the training set. 
Our method generalizes well to the testing cases in the FSC-147 dataset. Since the training and testing classes are disjoint, there are object placement patterns appearing only in the test set. We also show various examples of images from the web.
%We also show various examples of images that we collected with different object placement patterns. 
However, quantifying the exact extent of this generalization is non-trivial and we will state this clearly. %We believe that a large-scale dataset with diverse scenes, object types, and object placement patterns are necessary to investigate this further, which is unfortunately expensive to collect and annotate. 
\qu{\rthree}{Can the prototype handle object variations?} 
 %There is certainly a risk here. 
 There is indeed no guarantee.
 Ideally, the object prototype should be able to cover the object variations if there are sufficient training data for the generator. %Guaranteeing this is non-trivial and 
 We will add a new discussion to emphasize this point.


 \begin{table}[!ht] 
  \centering
  \vspace{-2mm}
\resizebox{0.4\textwidth}{!}{%
  \begin{tabular}{c|c|cc|cc}
    \toprule
    \multirow{2}{2cm}{Base Counter} & \multirow{2}{1cm}{Pseudo Masks} & \multicolumn{2}{c|}{Syn-multi} &  \multicolumn{2}{c}{Real-multi}  \\
    & & Val MAE &  Test MAE &  MAE & RMSE  \\
    \midrule
    \multirow{2}{1cm}{BMNet} & w/o & {32.39}  & {36.94} & {21.92} & {37.09} \\
   & w/ & \textbf{20.47} & \textbf{18.53} & \textbf{8.49} & \textbf{15.93} \\
  \midrule
  \multirow{2}{1.6cm}{SAFECount} & w/o & {22.58}  & {26.44} & {23.57} & {40.99} \\
   & w/ & \textbf{15.74} & \textbf{13.26} & \textbf{9.62} & \textbf{17.18} \\
  \midrule
  \multirow{2}{1cm}{Ours} & w/o & {32.46}  & {42.22} & {24.68} & {41.70} \\
   & w/ & \textbf{14.34} & \textbf{11.13} & \textbf{6.97} & \textbf{13.03} \\
    \bottomrule
  \end{tabular}}  
  \caption{ Performance of different counting methods with and without our proposed segmentation model.
  }\label{tab:generalization}  \vspace{-4.5mm}
\end{table}

==> table_before_change.tex <==

\begin{table*}[!ht] 
  \centering
\resizebox{0.8\textwidth}{!}{%
  \begin{tabular}{l|c|cc|cccc}
    \toprule
   \multirow{2}{*}{Method} & Training & \multicolumn{2}{c|}{Multi Set} & \multicolumn{4}{c}{Single Set} \\
    & Set & Test MAE & Test RMSE & Val MAE & Val RMSE & Test MAE & Test RMSE   \\
    \midrule
    \multirow{2}{*}{BMNet+} & Single & {25.55} & {40.35} & 15.74 & 58.53 & 14.62 & 91.83 \\
    & Single+Syn-multi & 11.44  & {23.22} & 24.24 & 73.42 & 20.89 & 99.04 \\
    \midrule
    \multirow{2}{*}{FamNet+ \cite{Ranjan2021LearningTC}} & Single & {19.42} & {39.78} &  23.75 & 69.07 & 22.08 & 99.54 \\
     & Single+Syn-multi & {11.31} & {18.84} &   29.45 & 94.33 & 26.93 & 116.12 \\
     \midrule
     \multirow{2}{*}{SAFECount \cite{Ranjan2021LearningTC}} & Single & {23.57} & {40.99}  & 14.42 & 51.72 & 13.56 & 91.30 \\
     & Single+Syn-multi & {9.80} & {32.40}  &  27.65 & 58.01 & 27.24 & 100.55 \\
     \midrule
     Ours & Single+Syn-multi & 6.97 & 13.03 & 18.55 & 61.12 & 20.68 & 109.14 \\
     %\multirow{2}{*}{BMNet \cite{Shi2022SimiCounting}} & GT & {18.29} & {124.02} & 0.26 & 4.39  \\
     %& RPN & {37.26} & {108.54} & {0.42} & {5.43}  \\
     %\midrule
    %\multirow{2}{*} {BMNet+ \cite{Shi2022SimiCounting}} & GT & {14.68} & {91.74} & {0.27} & {6.57}  \\
     %& RPN & {35.15} & {106.07} & {0.41} & {5.28}  \\
    \bottomrule
  \end{tabular}} \\ \vspace{1mm}
  \caption{ Comparison with training other class-agnostic counting methods (BMNet+, FamNet+ and SAFECount) using our synthetic multi-class images. Although the counting error on the multi-class test set can be reduced, the performance on the single-class test set drops significantly for all three baseline methods. 
  }\label{tab:concat_training} % \vspace{-2mm}
\end{table*}
